Learning to Place Guards by Reinforcement: A Geo-Free Neural Policy for the Vertex-Guard Art Gallery Problem

Neural combinatorial optimization (NCO) has shown that policies trained by reinforcement can construct strong solutions to NP-hard problems directly from raw instances. What such a policy actually learns, as opposed to what its decoder expresses, remains much less clear. We study this distinction on the vertex-guard Art Gallery Problem, the NP-hard task of choosing polygon vertices from which to observe an entire region. A pointer-network policy is trained from a coverage-aware reward over its own rollouts under the constraint we call geo-free inference: at test time it sees only vertex coordinates, with no visibility computation and no geometric oracle. The policy places guards economically but leaves a tail of under-covered polygons that widens far beyond the training range. To locate the cause, we freeze the trained encoder and read its embeddings with a small single-shot classifier, still geo-free at inference. The classifier closes most of the feasibility gap, in and out of distribution and at up to roughly five times the training range, cutting under-covered polygons by about an order of magnitude at an explicitly reported cost in guard count. We read this as evidence that the reinforcement-trained representation already encodes the geometry required for feasibility, and that residual failures reflect decoder calibration rather than missing knowledge. Probing a frozen encoder thus offers a practical way to ask what a neural combinatorial solver has internalized.

==> tables/tab_fixed_point.tex <==
% auto-generated by build_tables.py from data/setpred_iter_sweep.json
\begin{tabular}{lrrr}
  \toprule
  Inference passes $K$ & Mean $\mathrm{Cov}$ & Mean $|S|/n$ & Mean $|S|/\OPT$ \\
  \midrule
  $K=1$ & 0.9723 & 0.1968 & 1.2328 \\
  $K=2$ & 0.9712 & 0.1966 & 1.2302 \\
  $K=3$ & 0.9719 & 0.1966 & 1.2295 \\
  $K=5$ & 0.9719 & 0.1966 & 1.2292 \\
  \bottomrule
\end{tabular}

